A facility to Search for Hidden Particles (SHiP) at the CERN SPS

A new general purpose fixed target facility is proposed at the CERN SPS accelerator which is aimed at exploring the domain of hidden particles and make measurements with tau neutrinos. Hidden particles are predicted by a large number of models beyond the Standard Model. The high intensity of the SPS 400~GeV beam allows probing a wide variety of models containing light long-lived exotic particles with masses below ${\cal O}$(10)~GeV/c$^2$, including very weakly interacting low-energy SUSY states. The experimental programme of the proposed facility is capable of being extended in the future, e.g. to include direct searches for Dark Matter and Lepton Flavour Violation.

==> biblio/bib-bgtagger.tex <==

\bibitem{LS-LAB-PPO}
        M. Skorokhvatov et. al., 
        %``Liquid Scintillators Based on Linear Alkyl Benzene,'' 
        Doklady Physics, 2011, Vol. 56, No. 2, pp. 89–91.

%@article{Kraus:2006qp,
%      author         = "Kraus, C.",
%      title          = "{SNO with liquid scintillator: SNO+}",
%      collaboration  = "SNO+ Collaboration",
%      journal        = "Prog.Part.Nucl.Phys.",
%      volume         = "57",
%      pages          = "150-152",
%      doi            = "10.1016/j.ppnp.2005.12.001",
%      year           = "2006",
%      SLACcitation   = "%%CITATION = PPNPD,57,150;%%",
%}
%\cite{Kraus:2006qp}
\bibitem{Kraus:2006qp}
  C.~Kraus [SNO+ Collaboration],
  %``SNO with liquid scintillator: SNO+,''
  Prog.\ Part.\ Nucl.\ Phys.\  {\bf 57} (2006) 150.
  %%CITATION = PPNPD,57,150;%%
  %34 citations counted in INSPIRE as of 09 mar 2015

%article{Ding:2008zzb,
%      author         = "Ding, Yayun and Liu, Jinchang and Wang, Zhimin and Zhang,
%                        Zhiyong and Zhou, Pengju and others",
%      title          = "{A new gadolinium-loaded liquid scintillator for reactor
%                        neutrino detection}",
%      journal        = "Nucl.Instrum.Meth.",
%      volume         = "A584",
%      pages          = "238-243",
%      doi            = "10.1016/j.nima.2007.09.044",
%      year           = "2008",
%      SLACcitation   = "%%CITATION = NUIMA,A584,238;%%",
%}
%\cite{Ding:2008zzb}
\bibitem{Ding:2008zzb}
  Y.~Ding, J.~Liu, Z.~Wang, Z.~Zhang, P.~Zhou and Y.~Zhao,
  %``A new gadolinium-loaded liquid scintillator for reactor neutrino detection,''
  Nucl.\ Instrum.\ Meth.\ A {\bf 584} (2008) 238.
  %%CITATION = NUIMA,A584,238;%%
  %25 citations counted in INSPIRE as of 09 mar 2015

%@article{Back:2008zz,
%      author         = "Back, H.O. and Balata, M. and de Bari, A. and Beau, T.
%                        and de Bellefon, A. and others",
%      title          = "{Study of phenylxylylethane (PXE) as scintillator for low
%                        energy neutrino experiments}",
%      journal        = "Nucl.Instrum.Meth.",
%      volume         = "A585",
%      pages          = "48-60",
%      doi            = "10.1016/j.nima.2007.10.045",
%      year           = "2008",
%      SLACcitation   = "%%CITATION = NUIMA,A585,48;%%",
%}
%\cite{Back:2008zz}
\bibitem{Back:2008zz}
  H.~O.~Back, M.~Balata, A.~de Bari, T.~Beau, A.~de Bellefon, G.~Bellini, J.~Benziger and S.~Bonetti {\it et al.},
  %``Study of phenylxylylethane (PXE) as scintillator for low energy neutrino experiments,''
  Nucl.\ Instrum.\ Meth.\ A {\bf 585} (2008) 48.
  %%CITATION = NUIMA,A585,48;%%
  %12 citations counted in INSPIRE as of 09 mar 2015

%@article{Alimonti:2000xc,
%      author         = "Alimonti, G. and others",
%      title          = "{Science and technology of BOREXINO: A Real time detector
%                        for low-energy solar neutrinos}",
%      collaboration  = "Borexino Collaboration",
%      journal        = "Astropart.Phys.",
%      volume         = "16",
%      pages          = "205-234",
%      doi            = "10.1016/S0927-6505(01)00110-4",
%      year           = "2002",
%      eprint         = "hep-ex/0012030",
%      archivePrefix  = "arXiv",
%      primaryClass   = "hep-ex",
%      SLACcitation   = "%%CITATION = HEP-EX/0012030;%%",
%}
%\cite{Alimonti:2000xc}
\bibitem{Alimonti:2000xc}
  G.~Alimonti {\it et al.}  [Borexino Collaboration],
  %``Science and technology of BOREXINO: A Real time detector for low-energy solar neutrinos,''
  Astropart.\ Phys.\  {\bf 16} (2002) 205
  [hep-ex/0012030].
  %%CITATION = HEP-EX/0012030;%%
  %234 citations counted in INSPIRE as of 09 mar 2015

%@article{Alimonti:2009zz,
%      author         = "Alimonti, G. and others",
%      title          = "{The liquid handling systems for the Borexino solar
%                        neutrino detector}",
%      collaboration  = "Borexino Collaboration",
%      journal        = "Nucl.Instrum.Meth.",
%      volume         = "A609",
%      pages          = "58-78",
%      doi            = "10.1016/j.nima.2009.07.028",
%      year           = "2009",
%      SLACcitation   = "%%CITATION = NUIMA,A609,58;%%",
%}
%\cite{Alimonti:2009zz}
\bibitem{Alimonti:2009zz}
  G.~Alimonti {\it et al.}  [Borexino Collaboration],
  %``The liquid handling systems for the Borexino solar neutrino detector,''
  Nucl.\ Instrum.\ Meth.\ A {\bf 609} (2009) 58.
  %%CITATION = NUIMA,A609,58;%%
  %29 citations counted in INSPIRE as of 09 mar 2015

%@article{Schulte:2013dza,
%      author         = "Schulte, Lukas and Voge, Markus and Hoffmann, Akos and
%                        B\"oser, Sebastian and K\"opke, Lutz and others",
%      title          = "{A large-area single photon sensor employing
%                        wavelength-shifting and light-guiding technology}",
%      year           = "2013",
%      eprint         = "1307.6713",
%      archivePrefix  = "arXiv",
%      primaryClass   = "astro-ph.IM",
%      SLACcitation   = "%%CITATION = ARXIV:1307.6713;%%",
%}
%\cite{Schulte:2013dza}
\bibitem{Schulte:2013dza}
  L.~Schulte, M.~Voge, A.~Hoffmann, S.~B\"oser, L.~K\"opke and M.~Kowalski,
  ``A large-area single photon sensor employing wavelength-shifting and light-guiding technology,''
  arXiv:1307.6713 [astro-ph.IM].
  %%CITATION = ARXIV:1307.6713;%%
  %3 citations counted in INSPIRE as of 09 mar 2015


\bibitem{bgtagger:WOM-masterthesis}
        Dustin Hebeker, 
        ``Development of a single photon detector with wavelength shifting and light guiding technology'', 
        master thesis, University of Bonn, 2014




==> biblio/bib-calo.tex <==

\bibitem{herab:2007}
  Avoni G. \etal,
``The electromagnetic calorimeter of the HERA-B experiment",
	Nucl.\ Instr.\ and Meth. A{\bf 580} (2007) 1209.

\bibitem{baz:1996}
  A. Bazilevsky \etal, ``Performance of the PHENIX EM Calorimeter",
IEEE Trans.\ on\ Nucl.\ Science {\bf 43} (1996) 1491.
	
\bibitem{lhcb:2010}
  Shopper A. \etal,
``Overview of the LHCb calorimeter system",
	Nucl.\ Instr.\ and Meth. A{\bf 623} (2010) 219.

\bibitem{geant4}	
S. Agostinelli \etal,
``Geant4 - a simulation toolkit", 
	Nucl.\ Instr.\ and Meth. A{\bf 508} (2003) 250;
J. Allison \etal, 
	``Geant4 developments and applications",
	IEEE Trans.\ on\ Nucl.\ Science {\bf 53} (2006) 270.

\bibitem{ecal:mapd}
	N. Antimov \etal, ``Beam test of Shashlyk EM calorimeter prototypes readout by novel MAPD
with super high linearity", 	Nucl.\ Instr.\ and Meth. A{\bf 617} (2010) 78;

		
\bibitem{ecal:digi}
	D. Hadley, ``Digital filtering performance in the ATLAS Level-1 Calorimeter Trigger",
IEEE Real Time Conference (2010), doi:10.1109/RTC.2010.5750349.
	
\bibitem{ecal:sampic}
	E. Delagnes, D. Breton, H. Grabas, J. Maalmi, P. Rusquart, et al, ``The SAMPIC Waveform
and Time to Digital Converter". 2014 IEEE Nuclear Science Symposium and Medical Imaging Conference (2014 NSS/MIC), and 21st Symposium on Room-Temperature Semiconductor X-Ray and Gamma-Ray Detectors, Nov 2014, Seattle, United States.


==> biblio/bib-computing.tex <==

\bibitem{computing:FairRoot}
        http://fairroot.gsi.de

\bibitem{computing:FAIR}
        http://www.fair-center.eu

\bibitem{computing:ALICE-O2}
        http://iopscience.iop.org/1742-6596/513/1/012037

\bibitem{computing:ROOT}
        Rene Brun and Fons Rademakers, 
        ROOT - An Object Oriented Data Analysis Framework, 
        Proceedings AIHENP'96 Workshop, Lausanne,
        Sep. 1996, Nucl. Inst. \& Meth. in Phys. Res. A 389 (1997) 81-86.
        See also http://root.cern.ch/.

\bibitem{computing:github}
        https://github.com/ShipSoft
                
\bibitem{computing:docker}
        https://www.docker.com
        
\bibitem{computing:yarn}
        http://hadoop.apache.org/docs/stable/index.html
        

        


==> biblio/bib-facility.tex <==

\bibitem{Ferrari:2005zk}
  A.~Ferrari, P.~R.~Sala, A.~Fasso and J.~Ranft,
  ``FLUKA: A multi-particle transport code,''  CERN-2005-010 (2005).  

%\cite{Bohlen:2014}
\bibitem{Bohlen:2014} 
 T.T.~B{\"o}hlen et al., %F.~Cerutti, M.P.W.~Chin, A.~Fassò, A.~Ferrari, P.G.~Ortega, A.~Mairani, P.R.~Sala, G.~Smirnov and V.~Vlachoudis,
  ``The FLUKA Code: Developments and Challenges for High Energy and Medical Applications,''  Nuclear Data Sheets 120, 211-214 (2014).  

%\cite{Strabel:2015}
\bibitem{Strabel:2015}
C. Strabel, H. Vincke, "Radioation protection studies for the SHiP facility," CERN-RP-2015-020-REPORTS-TN, EDMS 1490910 (2015).

%\cite{FWirth:2006}
\bibitem{FWirth:2006}
D. Forkel-Wirth, "Zonage radiologique du CERN," EDMS 810149 (2006).

%\cite{Strabel:2014}
\bibitem{Strabel:2014}
C. Strabel, Heinz Vincke, K. Zabrzycki, "Radiation Protection studies for the CERN Neutrino Facility (CENF)," CERN-RP-2014-094-REPORTS-TN, EDMS 1427729 (2014).

%\cite{Vojtyla:2013}
\bibitem{Vojtyla:2013}
P. Vojtyla et al., "CENF radiological environmental considerations," Technical Note, EDMS 1427092 (2014).

%\cite{Cite:2014}
\bibitem{Cite:2014}
 "Prestations sur le Site du CERN," PSO/2011-011/Rev.5, EDMS 1155899 (2014).

%\cite{Survey:2013}
\bibitem{Survey:2013}
Y. Pira, A. Herve, "Survey radiologique septembre 2013 des zones TDC2/TCC2," EDMS 1319078 (2013).


\bibitem{magnet}
http://cds.cern.ch/record/711814/files/open-2004-003.pdf


==> biblio/bib-intro.tex <==

\bibitem{Dupont:2014}
  Dupont \etal,
  %``Penguins in their natural environment''
  Eur.\ Phys.\ J.\  C {\bf XX} (2014) XXX
  [arXiv:XXXX.XXXX [hep-ph]].
  %%CITATION = %%

\bibitem{NA62-TD} NA62 COLLABORATION; F. Hahn et al. NA62 Technical Design Document. NA62-10-07, CERN, 2010, 414 pp.
 NA62-10-07, https://cds.cern.ch/record/1404985.

\bibitem{NA62-status} NA62 COLLABORATION; F. Ambrosino et al. NA62 Status Report. CERN-SPSC-2007-035.



==> biblio/bib-muon.tex <==
\bibitem{Michael:2008bc} D. G. Michael et al, Nucl. Instr.  Meth. A596 (2008) 190.  
\bibitem{McFarland:2006pz}D.~Drakoulakos et al., hep-ex/0405002; K.S.~McFarland, Nucl. Phys. Proc. Suppl. 159 (2006) 10. 
\bibitem{Abe:2010gxa} ''Belle II Technical Design Report'', arXiv:1011.0352. 
\bibitem{Abe:2011ks}K.~Abe et al.,(T2K collaboration)  Nucl.Instrum.Meth. A659 (2011) 106-135; arXiv:1106.1238v2 [physics.ins-det].
%\bibitem{renker}D.~Renker and E.~Lorenz, JINST 4 (2009) P04004.
%\bibitem{nd280}Yu. Kudenko,  Nucl. Instr.  Meth. A598 (2009) 289.
%%CITATION = NUIMA,A598,289;%%

%\cite{Abe:2011ks}
%\bibitem{mppc} MPPC  (Multi-Pixel Photon Counter) is the trademark of HAMAMATSU PHOTONICS K. K. for  multi-pixel Geiger mode  avalanche photodiodes; 
%%CITATION = NONE;%%
%M.~Yokoyama  et al.,  Nucl. Instr.  Meth. A610 (2009) 128; 
%\cite{Yokoyama:2008hn}
%A.~Vacheret et al., Nucl.Instrum.Meth. A656 (2011) 69.
%\cite{Vacheret:2011zz}

\bibitem{Kudenko:2001qj}Y.~Kudenko et al., Nucl. Instr.  Meth. A469 (2001) 340.
%%CITATION = NUIMA,A469,340;%%
%\bibitem{smrd}O.~Mineev et al., Nucl. Instr.  Meth. A577 (2007) 540. 
%%CITATION = NUIMA,A577,540;%%
%\bibitem{smrd-1} S.Aoki et al., Nucl.Instrum.Meth. A698 (2013) 135.


\bibitem{Grauges:2010fi}
  SuperB Collaboration, ``SuperB Progress Reports - Detector'', arXiv:1007.4241.

\bibitem{muon:fluka}
 The FLUKA Monte Carlo, {http://www.fluka.org}.

\bibitem{Balbi:2014saa}
Balbi C. \etal,
``Test and simulation of plastic scintillator strips readout by silicon photomultipliers'',
Journal of Instrumentation, vol. 9 (2014).

\bibitem{muon:nicadd}
FNAL NICADD Photoinjector Laboratory, {http://nicadd.niu.edu/fnpl/}.

\bibitem{muon:bicron}
Bicron specs,  {http://www.detectors.saint-gobain.com/fibers.aspx}.

\bibitem{muon:kuraray}
Kuraray Plastic Scintillating Fibers, {http://kuraraypsf.jp/psf}.

\bibitem{Ivashkin:1997sa}
A. Ivashkin, Y. Kudenko, O. Mineev and J. Imatato,
`` Scintillation ring hodoscope with WLS fiber readout'', 
Nucl.\ Instr. and Meth. A {\bf 394} (1997).

\bibitem{PlaDalmau:2000bf} 
A. Pla-Dalmau, A. D. Bross and K. L. Mellott, ``Low-cost extruded plastic scintillator'', 
Nucl.\ Instr.\ and Meth. A {\bf 466} (2001).

\bibitem{muon:nicadd2}
A. Pla-Dalmau, A. D. Bross and V. V. Rykalin, 
``Extruding plastic scintillator at Fermilab'', 
Nuclear Science Symposium and Medical Imaging Conference (NSS/MIC), 2003 IEEE, (2003).

\bibitem{muon:nicadd3} 
A. Dyshkant, V. Rykalin, A. Pla-Dalmau and D. Beznosko, 
``Extruded scintillator for the calorimetry applications'', AIP conference proceedings (2006) 867.



==> biblio/bib-nutaudet.tex <==
\bibitem{DONUT_Tau} K. Kodama {\it et al.} (DONUT Coll.), Phys. Lett. B504 (2001) 218

\bibitem{bopera}
The OPERA collaboration, \emph{The OPERA experiment in the CERN 
to Gran Sasso neutrino beam}, 2009 JINST 4 (P04018)

\bibitem{OPERA_tau1} N. Agafonova {\it et al.} (OPERA Coll.), Phys. Lett. B691 (2010) 138. 
\bibitem{OPERA_tau2} N. Agafonova {\it et al.} (OPERA Coll.), J. High Energy Phys. 11 (2013) 036.
\bibitem{OPERA_tau3} N. Agafonova {\it et al.} (OPERA Coll.), Phys. Rev. D 89 (2014)  051102 (R). 
\bibitem{OPERA_tau4} N. Agafonova {\it et al.} (OPERA Coll.), Prog. Theor. Exp. Phys. (2014) 101C01.  
 

\bibitem{OPERA_Film} T. Nakamura {\it et al.} Nucl. Instrum. Meth. A556 (2006) 80

\bibitem{CHORUS_Film} S. Aoki {\it et al.} Nucl. Instrum. Meth. A447 (2000) 361

%\bibitem{ECC} 

\bibitem{MCS} N. Agafonova {\it et al.}  (OPERA Coll.), New J. Phys. 14 (2012) 013026 

\bibitem{operanue} N. Agafonova  {\it et al.}  (OPERA Coll.), J. High Energy Phys. 7 (2013) 004. 

\bibitem{ELE-PI} L. Arrabito {\it et al.} (OPERA Coll.), JINST 2 (2007) P02001 

\bibitem{LEAD} A. Anokhina {\it et al.} (OPERA Coll.), JINST 3  (2008) P07002 

\bibitem{ces} C. Fukushima {\it et al.}, NIM A 592 (2008) 56.

\bibitem{NIWA} K. Niwa, K. Hoshino, K. Niu, Proc. Int. Cosmic  Ray. Symp. on High Energy Phenomena (1974) 149

\bibitem{S-UTS} K. Morishima and T. Nakano, JINST 5 (2010) P04011

\bibitem{TS} S. Aoki {\it et al.}, Nucl. Instrum. Meth B 51 (1990) 466

\bibitem{ESS_hard} N. Armenise {\it et al.}, Nucl. Instrum. Meth A551 (2005)  261. 
\bibitem{ESS_soft} L. Arrabito {\it et al.},  Nucl. Instrum. Meth  A568 (2006) 578.
\bibitem{ESS_track}  L. Arrabito {\it et al.}, JINST 2 (2007) P05004.
\bibitem{ESS_prec} M. De Serio {\it et al.}, Nucl. Instrum. Meth. A554 (2005) 247.

\bibitem{SySal} G. Rosa {\it et al.}, Nucl. Instrum. Meth. A 394 (1997) 357

\bibitem{ESS-INFR} C. Bozza {\it et al.}, Nucl. Instrum. Meth.  A 703 (2013) 204

\bibitem{PlCh} S. Balestra {\it et al.}, Nucl. Instrum. Meth. A 716 (2013) 96

\bibitem{lasso} A.~Alexandrov {\it et al.}, JINST 9 (2014) C02034. 


\bibitem{nutaudet:SciFiTrackerTDR}
        http://cds.cern.ch/record/1647400?ln=en
        
\bibitem{nutaudet:SciFiTracker} B. Beischer {\it et al.}, Nucl. Instrum. Meth. A 622 (2010) 542


\bibitem{ref:TOSCA} OPERA-3d OPERA-2d and TOSCA are products by Vector
Field Ltd., Oxford, UK (www.vectorfields.co.uk).

\bibitem{ref:balli} 
G. Di Iorio, B. Dulach, M. Incurvati et al., \emph{Ballistic techniques for
magnetic field calibration of large iron detectors operating in underground
areas}, 2003 Nuclear Physics B (Proc. Suppl.) 125 27-31.

\bibitem{ref:Bmeas} 
A. Cazes, A. Cecchetti, B. Dulach et al., \emph{Electromagnetic 
characterization of the 990 ton gapless magnets of the OPERA experiment}, 
2007 JINST 2 (T03001).

\bibitem{sauli} F.Sauli, Nucl. Instr. and Meth. A 386 (1997) 531.
\bibitem{kloe2} A.~Balla {\it et al.}, Nucl. Instr. and Meth. A 732 (2013) 221.
\bibitem{gigi} G.~Cibinetto, private communication.
\bibitem{BLIND-GEM} M. Alfonsi et al., {\it Performance measurements on closed-geometry GEM like detectors}, presented at the MPGD2009 - 1st International Conference on Micropattern Gaseous Detectors, 12-15 June 2009  - Crete.
\bibitem{croci} G. Croci, {\it Development and characterization of Micro-Pattern Gaseous Detectors for HEP applications and beyond}, Ph.D Thesis, XXIII cycle (2010), University of Siena.
\bibitem{breskin2} L. Arazi et al., {\it Beam studies of the Segmented Resistive WELL: a potential thin sampling element for Digital Hadronic Calorimetry}, Nucl. Inst. \& Meth. {\bf A 732} (2013) 199.
\bibitem{GEM1} F. Sauli, {\it GEM: A new concept for electron amplification in gas detectors.}, Nucl. Inst. \& Meth. {\bf A 386} (1997) 531.
\bibitem{MM1} I. Giomataris et al., {\it Micromegas: a high-granularity, position sensitive gaseous detector for high particle flux environments.}, Nucl. Inst. \& Meth. {\bf A 376} (1996) 29.
\bibitem{Pestov} Y. Pestov et al., {\it A spark counter with large area}, Nucl. Instr. \& Meth. {\bf 93} (1971) 269.
\bibitem{santo} R. Santonico, R. Cardarelli, {\it Development of Resistive Plate Counters}, Nucl. Instr. \& Meth. {\bf A 377} (1981) 187.
\bibitem{bencivenni} M. Anelli et al., {\it Glass electrode spark counters}, Nucl. Instr. \& Meth. {\bf A 300} (1991) 5072.
\bibitem{rui2} G. Bencivenni, R. De Oliveira, {Private communication} (2014).
\bibitem{moreira} M.J. French et al, Nucl. Instr. and Meth. A 466 (2001) 359-365.


\bibitem{bsant}
R. Santonico and R. Cardarelli, \emph{Development of resistive plate counters}, NIMA 187 (1981), 377 \\
R. Santonico, R. Cardarelli et al., \emph{Progress in resistive plate counters}, NIMA 263 (1988), 20 

\bibitem{newRPC}
L. Paolozzi et al., \emph{Test for upgrading the RPCs at very high couting 
rate}, PoS(RPC2012) 065. 

\bibitem{rpc_newgas}  
R. Cardarelli et al., \emph{New RPC gas mixtures for large area apparatuses}, 
2014 JINST 9 (C11003).

\bibitem{OPERAcs}
A. Paoloni, \emph{The OPERA RPC system}, 2014 JINST 9 (C10003).

\bibitem{OPERAgas}
A. Paoloni et al., \emph{Gas mixture studies for streamer operation of Resistive Plate Chambers at low rate}, NIMA 583 (2007), 264.

\bibitem{rpc_recover} F. Ferroni, 
\emph{The second generation Babar RPCs: Final evaluation of performances}, 
NIMA 602 (2009), 649.

\bibitem{OPERAQC}
A. Paoloni et al., \emph{Tests on OPERA RPCs}, Nuclear Physics B (Proc. Suppl.), 158 (2006) 93.

\bibitem{buni1}{UNI 8457/87 and 8457/A1/96}

\bibitem{buni2}{UNI 9174/87 and 9174/A1/96}




==> biblio/bib-online.tex <==

\bibitem{LHCb-TDAQ-TDR:2014}
   LHCb collaboration,
   ``LHCb Trigger and Online Upgrade Technical Design Report''
   CERN-LHCC-2014-016 ; LHCB-TDR-016. 2014.


==> biblio/bib-physics.tex <==

\bibitem{DONUT:2008}
  K. Kodama \etal,
  Final tau-neutrino results from the DONuT experiment, 
  Phys. Rev. D 78 (2008) 052002.   

\bibitem{OPERA:2010}
  N. Agafonova \etal, 
  Observation of tau neutrino appearance in the CNGS beam with the OPERA experiment, 
  Prog. Theor. Exp. Phys. 10 (2014) 101C01. 




==> biblio/bib-req.tex <==


\bibitem{doublecharm} C. Lourenco, H.K. Wohri, Phys. Rept. {\bf 433} (2006) 127-180.

\bibitem{f_ds} JHEP {\bf 1309} (2013) 058.

\bibitem{pdg} PDG 2014.


==> biblio/bib-sensitivity.tex <==
%===========
% scalar portal:
%===========
\bibitem{Clarke:2013aya} 
J.~D.~Clarke, R.~Foot and R.~R.~Volkas, JHEP {\bf 02}, 123 (2014) [arXiv:1310.8042 [hep-ph]].

\bibitem{Batell:2009jf}
 B.~Batell, M.~Pospelov and A.~Ritz, Phys.Rev. D {\bf 83}, 054005 (2011) [arXiv:0911.4938 [hep-ph]].

\bibitem{Schmidt-Hoberg:2013hba}
[K.~Schmidt-Hoberg, F.~Staub and M.~W.~Winkler, Phys. Lett. {\bf B} 727, 506 (2013)
[arXiv:1310.6752 [hep-ph]].


\bibitem{Voloshin:1985tc} 
  M.~B.~Voloshin,
  Sov.\ J.\ Nucl.\ Phys.\  {\bf 44}, 478 (1986)
  [Yad.\ Fiz.\  {\bf 44}, 738 (1986)].
  %%CITATION = SJNCA,44,478;%%
  %134 citations counted in INSPIRE as of 06 Mar 2015

\bibitem{Raby:1988qf} 
  S.~Raby and G.~B.~West,
  %``The Branching Ratio for a Light Higgs to Decay Into $\mu^+ \mu^-$ Pairs,''
  Phys.\ Rev.\ D {\bf 38}, 3488 (1988).




\bibitem{Truong:1989my} 
  T.~N.~Truong and R.~S.~Willey,
  %``Branching Ratios for Decays of Light Higgs Bosons,''
  Phys.\ Rev.\ D {\bf 40}, 3635 (1989).
  %%CITATION = PHRVA,D40,3635;%%
  %14 citations counted in INSPIRE as of 06 mar 2015

\bibitem{Donoghue:1990xh} 
  J.~F.~Donoghue, J.~Gasser and H.~Leutwyler,
  %``The Decay of a Light Higgs Boson,''
  Nucl.\ Phys.\ B {\bf 343}, 341 (1990).

%\bibitem{Lourenco}
%C.~Lourenco, H.~K.~Wohri, Phys. Rept {\bf 433}, 127 (2006).

\bibitem{Wei:2009zv}
  J.-T.~Wei and others [BELLE Collaboration],  
Phys.\ Rev.\ Lett. {\bf 103}, 171801 (2009)
[arXiv:0904.0770 [hep-ex]].

\bibitem{Aubert:2008ps}
B.~Aubert and others [Babar Collaboration],
Phys.\ Rev.\ Lett. {\bf 102}, 091803 (2009)
[arXiv:0807.4119 [hep-ex]].
  
\bibitem{Chen:2007zk}
K.-F.~Chen and others [BELLE Collaboration],
Phys.\ Rev.\ Lett. {\bf 99}, 221802 (2007)
[arXiv:0707.0138 [hep-ex]].

\bibitem{delAmoSanchez:2010bk}
P.~del Amo Sanchez and others [Babar Collaboration]
Phys.\ Rev. D {\bf 82}, 112002 (2010)
[arXiv:1009.1529 [hep-ex]].

\bibitem{Bergsma:1985qz}
F.~Bergsma and others [CHARM Collaboration],
Phys.\ Rev. B {\bf 157}, 458 (1985).


\bibitem{bib:GorbShap2007}D.~Gorbunov and M.~Shaposhnikov, JHEP 0701 (2007) 015, arXiv:0705.1729 [hep-ph]
\bibitem{bib:CaneShap2010}L.~Canetti and M.~Shaposhnikov, JCAP 1009 (2010) 001 



==> biblio/bib-timing.tex <==


\bibitem{Hamamatsu_R13089} <http://www.hamamatsu.com/eu/en/product/category/3100/3001/R13089/index.html>


==> biblio/bib-tracker.tex <==
\bibitem{Makankin:2014}
 A.M. Makankin \etal, Nucl.\ Instr.\ and Methods in Phys.\ Res.\ A {\bf 735} (2014) 649-654.
See also developments for NA61/SHINE in section 2.7 of CERN-SPSC-2014-031.

%\bibitem{Movchan-PSD8} S. Movchan. Straw Tracker Prototype for the precise measurement of very rare decay. 
%8th. International Conference on Position Sensitive Detectors.
%Glasgow: PSD8. 2008. p. 307-309.
%\bibitem{Azorskiy} N.Azorskiy, S.Bazilev, L.Glonti et al.  Design and Test Results of NA62 Straw Detector First Prototype. 
%JINR P13-2013-50, Dubna, 2013, 18 pp.
%http://www1.jinr.ru/Preprints/2013/050(P13-2013-50).pdf
%\bibitem{Movchan-ISS} S.Movchan. NA62 straw tracker. The XII-th International School-Seminar.
%The Actual Problems of  Microworld Physics. Gomel, Belarus, July 22 - August
%2, 2013 http://gomelschool.hep.by/.
%\bibitem{Kolesnikov} A.Kolesnikov.  Automation of measurement systems and quality control of modules for 
%the CERN experiment NA62 manufactured by JINR. XXIV International
%Symposium on Nuclear Electronics \& Computing. BULGARIA, VARNA, 09-16 September, 2013 http://nec2013.jinr.ru/.
\bibitem{BRR} W. Blum, W. Riegler, L. Rolandi,  ``Particle Detection with Drfit Chambers'', 2nd edition, 2008, Springer.
\bibitem{GARFIELD} GARFIELD   ref
%http://cern.ch/magboltz   http://cern.ch/magboltz
%http://cern.ch/garfield   http://cern.ch/garfield
%http://cern.ch/garfieldpp http://cern.ch/garfieldpp
http://cern.ch/magboltz, 
http://cern.ch/garfield, 
http://cern.ch/garfieldpp. 
\bibitem{Eric_strawsimulnote} Eric vH's straw tracker simulation note.
\bibitem{CARIOCA} CARIOCA chip
\bibitem{ASDBLR} ``Radiation hardness: design approach and measurements of the ASDBLR ASIC for the ATLAS TRT'', 
   N. Dressnandt, M. Newcomer, O. Rohne, S. Passmore, 
   Nuclear Science Symposium Conference Record, 2002 IEEE, 
   10-16 Nov. 2002,  pp. 151 - 155 vol.1 
   ISBN 0-7803-7636-6.
   New ASDBLR chip:
  ``New Front-end Electronics for the Upgrade of the ATLAS Muon Drift Tube Chambers at High LHC Luminosity'',
  Philipp Schwegler et al., Proceedings of TWEPP 2013.
  %\url{http://indico.cern.ch/event/228972/session/9/contribution/102}
\bibitem{pythia8} PYTHIA 8
\bibitem{TemurEnik} Temur Enik, private communication.
\bibitem{LHCbUpgradeLOI} LHCb Upgrade LOI. 

%\bibitem{NA34} Bettoni $et$ $al.$, NIM A, 252, Issues 2–3, 1 December 1986, Pages 272–280.

% actually cited in Tracker.tex
%\cite{NA62-TD}).
%\cite{vessel:EoI}
%\cite{Eric_strawsimulnote}.
%\cite{GARFIELD}.
%\cite{BRR}.
%\cite{pythia8} 
%\cite{geant4}. 
%\cite{TemurEnik}. 
%\cite{CARIOCA}.  
%\cite{ASDBLR},
%\cite{LHCbUpgradeLOI}.
%\cite{Makankin:2014}. 



==> biblio/bib-vessel.tex <==

\bibitem{vessel:EoI}
        SHiP EoI

%\bibitem{bgtagger:WOMproposal}
         %L.~Schulte, M.~Voge, A.~Hoffmann, S.~B\"ose, L.~Kö\"op and M.~Kowalski,
         %``A large-area single photon sensor employing wavelength-shifting and 
         %  light-guiding technology,'' arXiv:1307.6713 [astro-ph.IM].





==> conclusions/Conclusions.tex <==
\chapter{Conclusions}
\label{sec:project}

% In order to take into account future extensions of the experimental programme, and re-use 
% of the facility, the proposed orientation of the beam line and the underground complex 
% allows reserving 100~m (CHECK WITH JOHN AND MARTIN) of space beyond the experimental hall
% which is currently free from important structures.


==> detector/Spectrometer.tex <==
\subsection{Spectrometer}

\label{sec:spectrometer}

\noindent The purpose of the HS spectrometer is to reconstruct with high efficiency the tracks
of charged particles from the decay of hidden particles, while rejecting background 
events. Additionally, the spectrometer must provide an accurate determination of the track 
momentum and of the flight direction within the fiducial decay volume. An associated timing
detector (Section~\ref{sec:timing_detectors}) must provide information on the coincidence of tracks combined into a vertex with 
very high timing accuracy in order to remove combinatorial background. 
The invariant mass, the vertex quality, the timing, and the pointing to the production target are crucial
tools for rejecting background from spurious $V^0$ meson decays or from random combinations. The 
bulk of the charged particles are expected to have momenta between a few ${\rm GeV}/c$ and 
$50~{\rm GeV}/c$, and polar angles peaking around 30~mrad, with a long tail to 300-400~mrad 
(see Figs. XXX and YYY, section XXX).\\

The spectrometer consists of a large aperture dipole magnet (\ref{sec:spectrometermagnet}) 
located between two tracking stations separated by 5m. Each tracking station consists of two 
straw tracking layers upstream of the magnet, and two straw tracking layers downstream 
(\ref{sec:tracker}).\\



==> nusensitivity/DarkMatter.tex <==


\subsection{Direct Dark Matter detection}

A rather systematic study of the detection of light dark matter produced via the dark photon portal 
has been performed in a number of papers \cite{Batell:2009di,Izaguirre:2013uxa,Batell:2014mga,Kahn:2014sra}.
The most stringent constraints follow from the highest POT experiment, LSND,  provided that the 
dark matter is within kinematic reach. A typical detection scheme in the proton beam dump experiments 
is built on the following chain of events: 
\begin{equation}
pp \to \pi^0 + X, ~~ \pi^0  \to A \gamma, ~~ A \to \chi\bar\chi, ~~ \chi ~ {\rm scattering~on~electrons/nuclei}
\end{equation}
where A is the dark photon and $\chi$ the darm matter particle.
%These results significantly constrain, but do not fully rule out, MeV-scale 
%dark matter models, suggested as a candidate explanation of the 511 keV excess from the galactic bulge. 
%Currently, the MiniBooNE collaboration is conducting a dedicated search for such states in a beam dump mode run~\cite{Dharmapalan:2012xp}. 
%The summary of the existing constraints on light dark matter 
%produced via vector portal is given in Fig. \ref{fig:VPfig6}. 
%Similar constraints were also derived for light dark 
%matter coupled to the SM via the baryonic vector portal \cite{Batell:2014yra}. It is important to emphasize that these constraints 
%cover the low mass region of parameter space inaccessible to traditional underground direct detection experiments. 


The experimental signature of dark matter interaction is  neutral current interaction in massive detector, both on electrons and on  nuclei.
The studies described in this section for the SHIP neutrino detector are based on the identification of scattering of dark matter particles on electrons. Scattering on nuclei could a subject for a future study.\\ 
To estimate the sensitivity  a model of kinetic mixing mediation was assumed\cite{Deniderville}and  signal distributions were calculated accordingly. \\ 
The main backgrounds for this search are similar to the search for the $\nu_\tau$ anomalous magnetic moment (see Section~\ref{MagMom}): neutral current $\nu_\mu$ and $\nu_e$ scattering on electrons, and charged current elastic, diffractive, resonant and deep inelastic  $\nu_e$ scattering on nuclei. \\
The GENIE MonteCarlo was used to generate the  background events. The main variables to separate signal from background are the electron energy and the angle with respect to the neutrino direction and the number of reconstructible particle at the neutrino interaction vertex. For this study we assumed that the SHIP neutrino detector is able to reconstruct charged pion and kaons and photons if above 100MeV and protons above 170MeV, assuming the neutrino  interaction occurs in  the lead plates. Due to the unknown creation point of the neutrino in the upstream target, the electron angle reconstruction is smeared   by about 1mrad, while it is assumed here, based on the OPERA experience, that the electron angle is reconstructed in the detector with a resolution of 3mrad, thereby dominating the total angular resolution. \\
Figure~\ref{fig:sig_DM} shows the correlation between the electron energy and the angle for signal candidates, in a model (a) with the dark photon of 800MeV of mass and the dark matter particle of 200MeV of mass and (b) with the dark photon of 405MeV of mass and the dark matter particle of 200MeV of mass. Most of the signal is concentrated at low energy, below 10-20GeV and with angles between 10mrad and  20mrad. \\
%These cuts are by no means optimised, Given we don't have simulated all possible combinations of dark photon and dark matter masses we consider this background estimate as an order of magnitude calculation and by no means a precise computation of the sensitivity.
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.35\linewidth]{../../neutrinos/ship_mv_800mev_mx_200mev.pdf}
\includegraphics[width=0.35\linewidth]{../../neutrinos/ship_mv_405mev_mx_200mev.pdf}
\caption{Electron scattering angle (mrad) vs.  electron energy (GeV) for signal candidates, (a) in a model with the dark photon of 800MeV of mass and the dark matter particle of 200MeV of mass and (b) with the dark photon of 405MeV of mass and the dark matter particle of 200MeV of mass.}
\label{fig:sig_DM}
\end{center}
\end{figure}
Figure~\ref{fig:bidi_DM} shows, for the  four neutrino scattering processes studied, for $\nu_e$ scattering, the correlation plots between the electron energy and the electron angle, with respect to the neutrino direction. 
These angular and energy cuts mentioned above are  applied to suppress the background. Table~\ref{tab:DM} shows, for the various background contributions, the number of expected events after cuts during the whole SHIP data-taking. The signal efficiency after cuts was estimated to be about 50\%.  Given we don't have simulated all possible combinations of dark photon and dark matter masses we consider this background estimate as an order of magnitude calculation and by no means a precise computation of the sensitivity. A more detailed analysis is left for future studies.
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.35\linewidth]{../../neutrinos/nuel.pdf}
\includegraphics[width=0.35\linewidth]{../../neutrinos/qel.pdf}\\
\includegraphics[width=0.35\linewidth]{../../neutrinos/res.pdf}
\includegraphics[width=0.35\linewidth]{../../neutrinos/dis.pdf}
\caption{Electron scattering angle vs.  electron energy  for elastic $\nu_e$ scattering on electrons, quasi-elastic, deep inelastic and  resonant scattering for candidates that have no reconstructible tracks associated the neutrino interaction vertex, as described in the text.}
\label{fig:bidi_DM}
\end{center}
\end{figure}

\begin{table}[H]
\begin{center}
\begin{tabular}{llllll}
\hline
                      	&     $\nu_e$   &      $\bar{\nu_e}$  & $\nu_\mu$  & $\bar{\nu_\mu}$    & all  \\
\hline
elastic scattering on $e^-$   & 16 & 2 & 20 & 18 & 56\\
quasi - elastic scattering  & 105 & 73&   & & 178 \\
resonant scattering  & 13& 27 & & & 40\\
deep inelastic scattering  &3 & 7& & & 10\\
\hline
total               & 137 & 109 & 20  &18  & 284\\
 
\end{tabular}
\label{tab:DM}
\caption{Number of  background events  to the dark matter search after cuts, from neutrino interactions, as described in the text, with 2$\cdot 10^{20}$ p.o.t.}
\end{center}
\end{table}

With this number of background events and the above mentioned signal efficiency, we can estimate the expected 90\% U.L. on dark matter signal (taking into account the dependence of $\varepsilon$ on the number of events with the fourth power), and is shown as red line in Figure~\ref{fig:VPfig6}. 
 The sensitivty is quite considerable and compares well with
previous experiments. 
\begin{figure}[H]
%\centerline{\includepdf[width=0.55\textwidth]{InvisibleAprimeBounds}}
\centerline{\includegraphics[width=0.55\textwidth]{../../neutrinos/sensi.pdf}}
\caption{SHiP sensitivty, as  90\% U.L. on dark matter signal, vs. dark photon mass $A$ with the neutrino detector  shown as a red line. The blue contour corresponds to the 10 events sensitivity. The other lines  give constraints on the scattering of the 
light dark matter produced in $e$ and $p$ collisions with fixed targets. $\alpha_D= 0.1$, $m_\chi = 200$ MeV. $\varepsilon$ is the coupling constant of the dark photon to the electromagnetic current. }
\label{fig:VPfig6}
\end{figure} 
An additional handle to suppress the background could come from studying the space distribution of the neutrino interaction vertex and will be a subject of future studies. \\
In addition, if one switches from A′ to a leptophobic mediator, such as those of $U(1)_B$ models\cite{deNiderville},
 the constraints from lepton-driven experiments (BaBar and E137) will be significantly relaxed, and
SHiP will produce a strong additional reach to LSND and MiniBooNE. 



==> nutaudet/Nutaudet.tex <==

\label{sec:nutaudet}

\subsection{Neutrino target}

	\subsubsection{Emulsion target}

		\paragraph{Nuclear emulsion films }

		\paragraph{Bricks}

		\paragraph{Compact emulsion spectrometer }
		
		\paragraph{Emulsion Scanning and Analysis }

		\paragraph{Target magnetisation }				

	\subsubsection{Target Tracker}

%		\paragraph{Scintillating fibre tracker}
                \input{nutaudet/SciFi_tracker.tex}

		\paragraph{GEM tracker }

		\paragraph{Micromegas tracker }

\subsection{Muon magnetic spectrometer}

	\subsubsection{Magnet} 
	
	\subsubsection{RPC tracking system}

	\subsubsection{Drift Tubes as precision tracking system}

\subsection{(Trigger and data analysis)}


==> nutaudet/SciFi_tracker.tex <==
\paragraph{Scintillating fibre tracker}
\label{sec:scifi_tracker}

%An important part of the hybrid $\tau$-neutrino detector is its tracker.
%The main role of the latter is to record the positions where the trajectories
%of $\tau$-lepton decay products cross the tracker active zone and the time of the event.
%This provides the so called "space-time stamp" and allows to associate in the off-line
%scanned data analysis a particular tracks inside the Emulsion Cloud Chamber with the tracks
%detected by the tracker and reconstruct the trajectory as shown in Fig.XX. \\

A highest spatial resolution option, proposed for the $\tau$-neutrino detector tracker, 
is the sub-detector based on scintillating fibres.
This technology is chosen as the baseline option for upgrade of the large downstream
tracker in LHCb experiment. A lot of R$\&$D studies have been performed for the LHCb
SciFi project at CERN, TU of Dortmund, RWTH of Aachen and NRC Kurchatov Institute.
The SHiP experiment could benefit from these studies to very large extend, in particular,
using many elements of the LHCb SciFi tracker design and already developed production
infrastructure. 
The detailed description of the LHCb SciFi tracker design is given in \cite{nutaudet:SciFiTrackerTDR}. \\

		%\vfill
\begin{figure}[tp]
\centering
\includegraphics[height=10cm]{nutaudet/FibreMatXsection.pdf}
\caption{Scintillating fibre ribbon cross-section.}\label{nutaudet:FibreMatXsection}
\end{figure}%
%

The main active element of the tracker is a fibre ribbon. Its cross-section is shown in Fig. \ref{nutaudet:FibreMatXsection}.
The ribbon consists of the 250 $\mu$m scintillating fibres arranged in 5-6 layers and bound together
by the epoxy bonding, impregnated with TiO$_2$, in a 132 mm wide and 2000 mm long fibre mat (512 fibres-wide)
for the horizontal plane, and 900 mm long for the vertical plane of a module. I the current design 12 SciFi
tracker modules of 50 mm thickness will be installed, alternating the ECC brick walls of the $\tau$-neutrino detector.  
The perpendicular layers of ribbons are glued to a composite carrier (holder) panels, made of a closed-cell
foam (i.e. Rohacell) or a honeycomb, and thin carbon fiber sheets. The scintillating fibres from Kuraray supplier,
type SCSF-78MJ with double cladding, are used in the LHCb SciFi; the same are a viable option for the SHiP
tracker. An alternative option could be the BCF-12 fibres from Saint-Gobain company. The light yield value
for these types of fibres is typically around 8000 photons/MeV. A nominal emission spectrum for the
SCSF-78MJ fibre extends from about 400 to 600 nm and peaks at 450 nm, with a bulk optical absorption length
greater than 3 m. These properties are more than sufficient to achieve an excellent tracking efficiency
with the proposed module design. \\

The module consists of 7 ribbons in horizontal direction, and 15 ribbons in vertical, placed orthogonally
to achieve the best track spatial resolution in both $X\&Y$ planes, Fig. \ref{nutaudet:SciFiNuTrackerModule}.
The resolution is estimated \cite{nutaudet:SciFiTracker} to be better that 70 $\mu$m for ribbons with 6 layers
(but worsens for a smaller number of layers). \\

%\vfill
\begin{figure}[tp]
\centering
\includegraphics[height=8cm]{nutaudet/SciFiNuTrackerModule.pdf}
\caption{Exploded view of the Scintillating Fibre Tracker module.}\label{nutaudet:SciFiNuTrackerModule}
\end{figure}%
%

Light detection is carried out by the SiPM chips. Two SiPM manufacturers, Hamamatsu 
and KETEK, have developed dedicated devices for the SciFi Tracker. These custom devices
provide high photon detection efficiency (PDE) in a large wavelength range, high reliability
and low cross-currents. The readout end-face of the module is polished, while mirror
is put on the opposite face. The SiPM photo sensors are connected directly to the 
readout side.
Each ribbon is readout by four 128 channel SiPM chips. The design of the readout
boxes should account for a lack of space in vertical direction and, hence, allow
a flexible connection to the module. The SiPM cooling is not so crucial for the SHiP
$\tau$-neutrino detector as it is for the LHCb SciFi tracker, where SiPM will operate
at -40$^o$ C with the thermal uniformity of about 1 degree C. The SiPM irradiation is
negligible in our case. However cooling option is still attractive with respect to its
utilization to reduce the SiPM dark noise. An actual temperature regime optimal 
for the tracker operation is to be determined.  \\





==> sensitivity/signal.tex <==




==> sensitivity/tauNeutrinos.tex <==

\section{Neutrino Physics}

\subsection{tau neutrinos}

\subsection{Charm production and HNL normalization}

==> tracking/sst.tex <==

The basic detector element is a drift tube.
The cathode is formed by a thin layer of copper and gold (50 and 20~nm in NA62)
deposited on a PET foil. 
The anode is a thin tungsten wire (e.g. 30~$\mu$m diameter) coated with gold.
The electrical properties of the drift tubes are defined by the metal coating.
In the currently assumed design, %with straw length $\ell=5$~m, 
the electrical properties are expected to be the following:
\begin{itemize}
 \item capacitance $C=9.6~$pF/m, inductance $L=1.16~\mu$H/m,
 \item straw resistance $R=R_{\rm wire} + R_{\rm tube}$, 
       $R_{\rm wire}\approx80~\Omega/$m, $R_{\rm tube}\approx35~\Omega/$m, $R\approx115~\Omega/$m,
 \item characteristic impedance $Z_0=\sqrt{L/C}=350~\Omega$,
 \item characteristic frequency $f_0=R/(2\pi L) = 16~$MHz,
 \item signal attenuation length at high frequencies $\lambda=2\,Z_0/R \approx 6~$m.
\end{itemize}
The value of the input impedance of the preamplifier is a compromise between a good straw impedance matching 
and small cross-talk. A lower value is advantageous, as it guarantees lower cross-talk 
and signal enhancement due to current increase during signal reflection on the low termination impedance.
The reflected signal, which returns after travelling to the far end of the straw,
is strongly attenuated and does not contribute significantly. % to the output. 
The shaping time should be short in order to get a response from the first primary cluster 
and thus a better time resolution, but should be sufficiently long to integrate further
clusters such that there is only a single output pulse per particle hit.
Assuming 0.3~mm average spacing between primary clusters, the shaping time should be 
much longer than 15~ns for a slow gas and 6~ns for a fast gas.

Detector and signal studies will be performed in order to define the specifications 
for the input impedance of the preamplifier, the shaping
time and the ion tail cancellation.

The tracker readout electronics is composed of an analog and a digital part. 
After analog processing of the wire signal, the arrival time of the
track signal is digitized and sent to the data acquisition system in the 
required format.


The tracker detector is a gaseous detector organized in four stations. 
The number of readout electronics channels is equal to the number of straws,
or double that amount in case double-sided readout is used or if the 
5~m long straws are split into $2\times2.5~$m straws.

The readout electronics modularity conforms with the straw mechanical fixation and gas 
distribution modularity. Following the implementation of the NA62 tracker, the
currently assumed modularity of the detector in terms of high voltage, gas supply and 
readout is 16 straws, which results in 2272 readout boards for the case of 36352 channels.
The readout board comprises the readout electronics, high voltage and gas connections and 
is connected to the straws via a flexible circuit.
Since the readout electronics is exposed to negligible
radiation levels, it can be directly located on the detector and no special 
radiation hard components are needed.

The general diagram of the tracker readout electronics is shown on the left side of Fig.~\ref{fig:straw-electronics}.

\begin{figure}[tbp]
 \centering
 \includegraphics*[width=0.49\textwidth]{tracking/straw-electronics-general-diagram.jpg}
 \includegraphics*[width=0.49\textwidth]{tracking/straw-electronics-functional-diagram.jpg}
 \caption{
  Left: The general diagram of the tracker readout electronics.
  Right: Functional diagram of the analog part of the readout electronics.
  }\label{fig:straw-electronics}
\end{figure}

%\mysubsubsection{Analog part of readout electronics}

The analog part of the readout electronics contains two stages.
The first stage amplifies and shapes the detector signal.
The second stage extracts timing information (a discriminator or digitizer). 
Some parameters will need to be configurable (like thresholds), 
other need only to be monitored (like power supply voltages). 
The parameters and functionalities of all functional blocks will be specified
on the basis of detector and signal simulation and test measurements. 

The requirements for the analog part are defined by the position resolution 
achievable with one signal wire, currently assumed to be 120~$\mu$m. 
%Requirements for the analog part come from the required track position resolution,
%currently assumed to be 120~$\mu$m. 
This information is extracted from the arrival time of the leading edge of the straws 
signal, which depends on the particle track distance from the anode wire. 
With a maximum drift distance of about 5~mm, i.e. an electron total drift time of about 150~ns, 
the minimum required drift time resolution would be 3-4~ns.
%\mycomment{This may change in the future}.


custom analog front-end chip -- either one built for another experiment or a newly
designed chip. Design specifications will be drawn based on the output from the detector
and signal studies. An investigation of the usability and availability of existing chips
will be carried out. A few examples are discussed in the following.

For the NA62 straw tracker the CARIOCA chip was used~\cite{CARIOCA}.  
This is an 8-channel Amplifier Shaper Discriminator developed for the LHCb muon chambers. 
It is implemented using the IBM 0.25~$\mu$m CMOS process.
Two time constants are used in the base line restoration, tailored for its specific application.
It may be used with negative or positive input signal polarity.
The ASIC might be suitable for SHiP.
However, this chip is no longer available in sufficient quantities for the SHiP straw tracker 
and cannot be remanufactured, due to the old technology.
Currently, there is no follow-up chip being developed.

Another candidate is the ASDBLR chip~\cite{ASDBLR}, designed in 2002 for the ATLAS TRT straw
detector and used also in the LHCb Outer Tracker (OT). 
The ASDBLR acronym stands for Amplifier Shaper Discriminator with Base Line Restoration.
It  has two thresholds and two discriminator structures.
The 8-channel ASIC is implemented in bipolar technology,  in the phased-out DMILL process.
Due to the decommissioning of the LHCb OT during LHC Long Shutdown 2, several thousand chips 
may become available in 2018, probably enough to read out more than 40'000 electronics channels.
Although, the current OT digital part is not compatible with the current SHiP proposal,
new FPGA-based digitizer boards were developed at NIKHEF when the straw tube technology
was still being considered for the LHCb upgrade.
Their design is compatible with the SHiP electronics architecture and first prototypes
were already produced.

Parameters and requirements for the analog power regulators (voltages,
currents, stability, noise) will be defined upon analog front-end electronics design.
Parameters of the analog power supply will be monitored via the Experimental Control System
(ECS) interface, e.g. I2C.


The timing information is extracted from the signal shape, e.g. from the arrival time of the leading edge 
of the straw signal with respect to a master clock. The required drift time resolution is 
3-4 ns and a single-ended straw readout will be sufficient to achieve this resolution. 
The extraction of timing information can be achieved in two different ways:
(a) by discrimination of the shaped straw signal,  followed by edge detection and time stamping
of the discriminator output pulse with sub-nanosecond resolution by TDC,
or (b) by fast sampling and digitization of the shaped straw signal,
followed by digital signal processing of the acquired samples to extract the 
timing information.

Currently, the first method (with TDC) seems the most realistic. %suitable.
 The TDC can be directly implemented in the digital part.
Multiple channel sub-nanosecond TDC was recently implemented in low-cost FPGA.
The second method will be tested in the laboratory and conclusions will be made 
about its applicability.


The digital part of the readout electronics must provide time stamps for the leading
edges of the straw signals, processing, zero suppression, formatting and transmission
of digital data to the DAQ system via Ethernet. 
It will also include interfaces to the TFC system for timing
and synchronization via optical link, and to the ECS for the control/monitoring
via Ethernet. 
The whole digital part of the readout electronics can be implemented in a single 
readout FPGA with high speed links. The optical transceivers and the Ethernet
physical layer chip will provide physical connections to the Online system.


